One Shot 3D Photography

3D photography is a new medium that allows viewers to more fully experience a captured moment. In this work, we refer to a 3D photo as one that displays parallax induced by moving the viewpoint (as opposed to a stereo pair with a fixed viewpoint). 3D photos are static in time, like traditional photos, but are displayed with interactive parallax on mobile or desktop screens, as well as on Virtual Reality devices, where viewing it also includes stereo. We present an end-to-end system for creating and viewing 3D photos, and the algorithmic and design choices therein. Our 3D photos are captured in a single shot and processed directly on a mobile device. The method starts by estimating depth from the 2D input image using a new monocular depth estimation network that is optimized for mobile devices. It performs competitively to the state-of-the-art, but has lower latency and peak memory consumption and uses an order of magnitude fewer parameters. The resulting depth is lifted to a layered depth image, and new geometry is synthesized in parallax regions. We synthesize color texture and structures in the parallax regions as well, using an inpainting network, also optimized for mobile devices, on the LDI directly. Finally, we convert the result into a mesh-based representation that can be efficiently transmitted and rendered even on low-end devices and over poor network connections. Altogether, the processing takes just a few seconds on a mobile device, and the result can be instantly viewed and shared. We perform extensive quantitative evaluation to validate our system and compare its new components against the current state-of-the-art.

==> figures/farbrausch_scheme.tex <==
\begin{figure}
\centering%
\includegraphics[width=\linewidth]{figures/farbrausch_scheme.png}\\
\caption{Farbrausch network schematics \unsure{Not the real network, just a stand-in figure!}.}
\label{fig:fr_scheme}
\end{figure}


==> figures/inpainting_network.tex <==



\begin{tikzpicture}
\tikzstyle{connection}=[ultra thick,every node/.style={sloped,allow upside down},draw=\edgecolor,opacity=0.7]
\tikzstyle{copyconnection}=[ultra thick,every node/.style={sloped,allow upside down},draw={rgb:blue,4;red,1;green,1;black,3},opacity=0.7]

\pic[shift={(0,0,0)}] at (0,0,0)
    {Box={
        name=en0,
        caption= ,
        fill=ImgColor,
        opacity=1,
        height=32.0,
        width=0.046875,
        depth=40
        }
    };

\pic[shift={(0.5, 0, 0)}] at (en0-east)
    {Box={
        name=en1,
        caption= ,
        fill=ConvReLUColor,
        opacity=1,
        height=25.6,
        width=0.375,
        depth=25.6
        }
    };

\pic[shift={(0.5, 0, 0)}] at (en1-east)
    {Box={
        name=en2,
        caption= ,
        fill=ConvBNReLUColor,
        opacity=1,
        height=20.48,
        width=0.75,
        depth=20.48
        }
    };

\pic[shift={(0.5, 0, 0)}] at (en2-east)
    {Box={
        name=en3,
        caption= ,
        fill=ConvBNReLUColor,
        opacity=1,
        height=16.384,
        width=1.25,
        depth=16.384
        }
    };

\pic[shift={(0.5, 0, 0)}] at (en3-east)
    {Box={
        name=en4,
        caption= ,
        fill=ConvBNReLUColor,
        opacity=1,
        height=13.1072,
        width=3.0,
        depth=13.1072
        }
    };

\pic[shift={(0.5, 0, 0)}] at (en4-east)
    {Box={
        name=en5,
        caption= ,
        fill=ConvBNReLUColor,
        opacity=1,
        height=10.48576,
        width=8.0,
        depth=10.48576
        }
    };

\pic[shift={ (0.5,0,0) }] at (en5-east)
    {Box={
        name=pool5,
        caption= ,
        fill=UnpoolColor,
        opacity=1,
        height=13.1072,
        width=8.0,
        depth=13.1072
        }
    };

\pic[shift={ (0,0,0) }] at (pool5-east)
    {Box={
        name=copy5,
        caption= ,
        fill=CopyColor,
        opacity=1,
        height=13.1072,
        width=3.0,
        depth=13.1072
        }
    };

\path (en4-south) -- (en4-north) coordinate[pos=1.25] (en4-top) ;
\path (copy5-south)  -- (copy5-north)  coordinate[pos=1.25] (copy5-top) ;
\draw [copyconnection]  (en4-north)
-- node {\copymidarrow}(en4-top)
-- node {\copymidarrow}(copy5-top)
-- node {\copymidarrow} (copy5-north);

\pic[shift={(0.125,0,0)}] at (copy5-east)
    {Box={
        name=de5,
        caption= ,
        fill=ConvBNReLUColor,
        opacity=1,
        height=13.1072,
        width=3.0,
        depth=13.1072
        }
    };

\pic[shift={ (0.5,0,0) }] at (de5-east)
    {Box={
        name=pool4,
        caption= ,
        fill=UnpoolColor,
        opacity=1,
        height=16.384,
        width=3.0,
        depth=16.384
        }
    };

\pic[shift={ (0,0,0) }] at (pool4-east)
    {Box={
        name=copy4,
        caption= ,
        fill=CopyColor,
        opacity=1,
        height=16.384,
        width=1.25,
        depth=16.384
        }
    };

\path (en3-south) -- (en3-north) coordinate[pos=1.25] (en3-top) ;
\path (copy4-south)  -- (copy4-north)  coordinate[pos=1.25] (copy4-top) ;
\draw [copyconnection]  (en3-north)
-- node {\copymidarrow}(en3-top)
-- node {\copymidarrow}(copy4-top)
-- node {\copymidarrow} (copy4-north);

\pic[shift={(0.125,0,0)}] at (copy4-east)
    {Box={
        name=de4,
        caption= ,
        fill=ConvBNReLUColor,
        opacity=1,
        height=16.384,
        width=1.25,
        depth=16.384
        }
    };

\pic[shift={ (0.5,0,0) }] at (de4-east)
    {Box={
        name=pool3,
        caption= ,
        fill=UnpoolColor,
        opacity=1,
        height=20.48,
        width=1.25,
        depth=20.48
        }
    };

\pic[shift={ (0,0,0) }] at (pool3-east)
    {Box={
        name=copy3,
        caption= ,
        fill=CopyColor,
        opacity=1,
        height=20.48,
        width=0.75,
        depth=20.48
        }
    };

\path (en2-south) -- (en2-north) coordinate[pos=1.25] (en2-top) ;
\path (copy3-south)  -- (copy3-north)  coordinate[pos=1.25] (copy3-top) ;
\draw [copyconnection]  (en2-north)
-- node {\copymidarrow}(en2-top)
-- node {\copymidarrow}(copy3-top)
-- node {\copymidarrow} (copy3-north);

\pic[shift={(0.125,0,0)}] at (copy3-east)
    {Box={
        name=de3,
        caption= ,
        fill=ConvBNReLUColor,
        opacity=1,
        height=20.48,
        width=0.75,
        depth=20.48
        }
    };

\pic[shift={ (0.5,0,0) }] at (de3-east)
    {Box={
        name=pool2,
        caption= ,
        fill=UnpoolColor,
        opacity=1,
        height=25.6,
        width=0.75,
        depth=25.6
        }
    };

\pic[shift={ (0,0,0) }] at (pool2-east)
    {Box={
        name=copy2,
        caption= ,
        fill=CopyColor,
        opacity=1,
        height=25.6,
        width=0.375,
        depth=25.6
        }
    };

\path (en1-south) -- (en1-north) coordinate[pos=1.25] (en1-top) ;
\path (copy2-south)  -- (copy2-north)  coordinate[pos=1.25] (copy2-top) ;
\draw [copyconnection]  (en1-north)
-- node {\copymidarrow}(en1-top)
-- node {\copymidarrow}(copy2-top)
-- node {\copymidarrow} (copy2-north);

\pic[shift={(0.125,0,0)}] at (copy2-east)
    {Box={
        name=de2,
        caption= ,
        fill=ConvBNReLUColor,
        opacity=1,
        height=25.6,
        width=0.375,
        depth=25.6
        }
    };

\pic[shift={ (0.5,0,0) }] at (de2-east)
    {Box={
        name=pool1,
        caption= ,
        fill=UnpoolColor,
        opacity=1,
        height=32.0,
        width=0.375,
        depth=32.0
        }
    };

\pic[shift={ (0,0,0) }] at (pool1-east)
    {Box={
        name=copy1,
        caption= ,
        fill=CopyColor,
        opacity=1,
        height=32.0,
        width=0.046875,
        depth=32.0
        }
    };

\path (en0-south) -- (en0-north) coordinate[pos=1.25] (en0-top) ;
\path (copy1-south)  -- (copy1-north)  coordinate[pos=1.25] (copy1-top) ;
\draw [copyconnection]  (en0-north)
-- node {\copymidarrow}(en0-top)
-- node {\copymidarrow}(copy1-top)
-- node {\copymidarrow} (copy1-north);

\pic[shift={(0.125,0,0)}] at (copy1-east)
    {Box={
        name=de1,
        caption= ,
        fill=ConvColor,
        opacity=1,
        height=32.0,
        width=0.046875,
        depth=32.0
        }
    };

\end{tikzpicture}


==> figures/network_styles/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}


